Less is More: Selective Layer Finetuning with SubTuning

Finetuning a pretrained model has become a standard approach for training neural networks on novel tasks, resulting in fast convergence and improved performance. In this work, we study an alternative finetuning method, where instead of finetuning all the weights of the network, we only train a carefully chosen subset of layers, keeping the rest of the weights frozen at their initial (pretrained) values. We demonstrate that \emph{subset finetuning} (or SubTuning) often achieves accuracy comparable to full finetuning of the model, and even surpasses the performance of full finetuning when training data is scarce. Therefore, SubTuning allows deploying new tasks at minimal computational cost, while enjoying the benefits of finetuning the entire model. This yields a simple and effective method for multi-task learning, where different tasks do not interfere with one another, and yet share most of the resources at inference time. We demonstrate the efficiency of SubTuning across multiple tasks, using different network architectures and pretraining methods.

==> 2-NeurIPS/sections/acknowledgments.tex <==
\section{Acknowledgments}
We would like to thank Preetum Nakkiran, Asaf Noy, Asaf Maman and Itay Benou for comments on early version of the draft. GK is currently supported by a Simons Investigator Fellowship, NSF grant DMS-2134157, DARPA grant W911NF2010021,and DOE grant DE-SC0022199. GK is also grateful for support from Oracle Labs and past support by the NSF, as well as the Packard and Sloan foundations and the BSF.

==> 2-NeurIPS/sections/conclusions.tex <==
In this paper we introduced SubTuning, an efficient finetuning method that allows deployment of new tasks, without interfering with other tasks that share the same pretrained network. We showed that finetuning only a small subset of the network's layers can reach performance that is competitive with finetuning all the layers of the network, and in some cases can even drastically improve performance compared to full finetuning. This opens up a few promising directions for future research.

First, we note that in this work we studied selective finetuning of a subset of \emph{consecutive} layers. While this choice greatly simplifies our method, training a subset of non-consecutive layers can potentially improve performance even further. Therefore, an interesting direction for future work is to investigate the benefit from training arbitrary subsets of layers, as well as developing an algorithm for choosing the optimal subset.

Another promising direction for future research is to better understand the interplay between the architecture, the data, and the optimal subset of layers to be finetuned. As the study of the \emph{finetuning profiles} shows, different architectures and datasets can have different ``preferred'' layers for finetuning. In this paper, the method for choosing the best layer is simply to try all the options of consecutive subsets of layers. However, it might be possible to find measures, such as the gradient of the loss or the change in the weights during training, that can assist in choosing the correct subset, without performing a full training cycle for each subset.

==> 2-NeurIPS/sections/discussion.tex <==

 The wide adoption of neural networks for solving a multitude of tasks has drastically changed software development methodologies in AI-centric applications and products. More and more parts of the code are replaced by trained neural networks, instead of ``traditional'' algorithms. Some even predict that in many applications, all code will eventually be replaced by a single large neural network, completing the transition to Software 2.0 \cite{Karpathy_2017}.
 
While the benefits of embedding neural networks into the software stack are clear, this also poses some immediate challenges. In traditional software development, multiple teams can develop each part of the system independently from one another, where interfaces between parts of the code are clearly defined and conflicts can be safely handled by version control systems (e.g., git). When replacing software with learned networks, such independence is hard to maintain. Independent teams building a single network for solving different tasks need to coordinate a single training cycle each time a task is changed, and every task can negatively affect any other task. 


We believe that SubTuning can be a viable methodology for addressing this challenge. SubTuning allows developers to ``fork'' existing deployed networks and develop new tasks on top of the trained network, without interfering with the ``code'' of other teams that may also be using the network. This enables independent development of different tasks while maximizing performance, sharing of knowledge between tasks, and minimizing the computational cost of deploying new tasks. Thus, efficient finetuning methods like SubTuning can play a key role in transforming software development in the era of neural networks.



==> 2-NeurIPS/sections/extension_and_ablations.tex <==



In this section, we propose several enhancements to SubTuning, and also evaluate the significance of certain design choices. In Section~\ref{sec:siamese} we present an extension to SubTuning that combines the original network's features with newly finetuned layers, resulting in improved accuracy. In Section~\ref{sec:pruning}, we explore techniques to reduce the cost of SubTuning by implementing pruning, a process that removes unnecessary channels, without compromising much on performance.
Finally, in Section~\ref{sec:reinit}, we delve into the critical role of weight initialization in SubTuning. For the full experimental setup refer to Appendix~\ref{sec:experimental setup}.




\subsection{Siamese SubTuning} \label{sec:siamese}

In the MTL setting (Section \ref{sec:computationally_efficient_finetuning}), we assume that $f_\theta(\x)$ is already computed, and we want to minimize the cost of computing $f_{\tilde{\theta}}(\x)$, while preserving good performance. Since $f_\theta(\x)$ is computed anyway, its features are available at no extra cost\footnote{Neglecting the extra cost of the increased linear layer.}, and we can combine them with the new features. To achieve this, we concatenate the representations given by $f_\theta(\x)$ and $f_{\tilde{\theta}}(\x)$ before inserting them into the classification head. We call this method Siamese SubTuning.

We evaluated the effectiveness of Siamese SubTuning (See illustraion in \cref{fig:siamese_illustration} in Appendix~\ref{sec:app_siamese}) on multiple datasets and found it to be particularly beneficial in scenarios where data is limited. As demonstrated in Figure~\ref{fig:siamese}, when finetuning on 5,000 randomly selected training samples from the CIFAR-10, CIFAR-100, and Stanford Cars datasets, Siamese SubTuning with ResNet-18 outperforms standard SubTuning. It is worth noting that both SubTuning and Siamese SubTuning significantly improve performance when compared to linear probing in this setting. For instance, linear probing on top of ResNet-18 on CIFAR-10 achieves 79\% accuracy, where Siamese SubTuning achieves 88\% accuracy in the same setting. See also ResNet-50 results in Figure \ref{fig:siamese_resnet50} and Layer-wise (as opposed to block-wise) results are reported in Figure \ref{fig:siamese_full_layers} in the Appendix~\ref{sec:app_siamese}.

\subsection{SubTuning with Pruning}\label{sec:pruning}

\begin{figure}[h]
\centering
\hfill
\includegraphics[width=0.85\columnwidth,trim={0.5cm 0 0.5cm 0}]{2-NeurIPS/pruning_filtered.pdf}
\hfill
\caption{SubTuning with channel-wise pruning on the last 3 blocks of ResNet-50.
We plot the accuracy vs the pruning rate of different pruning techniques (Global vs. Local and pruning norm). The figure shows the best values for each parameter fraction.}
\label{fig:pruning}
\end{figure}

So far, we demonstrated the effectiveness of SubTuning in reducing the cost of adding new tasks for MTL while maintaining high performance on those tasks. To further optimize computational efficiency and decrease the model size for new tasks, we propose utilizing channel pruning on the SubTuned component of the model. We employ two types of pruning, local and global pruning, to reduce the parameter size and runtime of the model while preserving its accuracy. Local pruning removes an equal portion of channels for each layer, while global pruning eliminates channels across the network disregarding how many channels are removed per layer. Similar to \citet{pruning}, for both pruning techniques we prune the weights with the lowest L1 and L2 norms so that we can meet the target pruning ratio. 

In \cref{fig:pruning} we illustrate the effectiveness of combining channel pruning with SubTuning on the last 3 blocks of ResNet-50. Instead of copying the weights and then training the blocks, as we have done so far, we add an additional step of pruning before the training. This way we only prune the original, frozen, network once for all future tasks.
Our results show that pruning is effective across different parameter targets, reducing the cost with only small performance degradation. For example, when using less than 3\% of the last 3 blocks (about 2\% of all the parameters of ResNet-50) we maintain 94\% accuracy on the CIFAR-10 dataset. In the same setting, linear probing gets about 91\% accuracy. For more pruning results see Figure~\ref{fig:pruning_full} in the Appendix.

\subsection{Effect of Random Re-initialization}\label{sec:reinit}
We now show that initializing the weights of a model with the pretrained weights from a different task improves the performance and speed of training when SubTuning it on a new task. Specifically, in \cref{fig:reinit_10-80e} (in the Appendix) we finetune ResNet-50 pretrained on ImageNet, on the CIFAR-10 dataset. We compare this to randomly reinitializing the weights and show that, similar to standard finetuning, the pretrained weights led to a significant improvement in performance and faster convergence. We also find that the earlier the layers we finetuned, the greater the improvement is. This study demonstrates that using pretrained weights as initialization for SubTuning can lead to faster and better results.
We note that even with longer training time of 80 epochs, random initialization achieves poor performance.
% To refute the hypothesis that randomly initialized SubTuning performs poorly due to lack of training, we also ran an 80 epoch run without significant performance gains.


==> 2-NeurIPS/sections/introduction.tex <==

\begin{figure}[ht!]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[trim={0.5cm 0.1cm 0.5cm 0.1cm}, clip,width=\textwidth]{2-NeurIPS/FineTuning.png}
    \end{minipage}
    \hfill \rule[0.5cm]{0.48\textwidth}{0.3pt} 
    \begin{minipage}{0.48\textwidth}
        \centering
    %\vspace{-0.4cm}
    \includegraphics[trim={0.5cm 0.1cm 0.5cm 0.1cm}, clip,width=\textwidth]{2-NeurIPS/LinearProbing.png}
    \end{minipage}
    \hfill \rule[0.5cm]{0.48\textwidth}{0.3pt} 
    % \vspace{-0.4cm}
    \begin{minipage}{0.48\textwidth}
        \centering
        %\vspace{-0.4cm}
        \includegraphics[trim={0.5cm 0.1cm 0.5cm 0.1cm}, clip,width=\textwidth]{2-NeurIPS/SubTuning.png}
    \end{minipage}
    \caption{Illustration of finetuning, linear probing and SubTuning in a multi-task setting. In SubTuning we train only a subset of intermediate layers for each task. At inference time, the early layers are shared between all tasks while the tuned layers (green and red) are separate for each task. The output maps of the tuned layers are concatenated in the ``batch'' axis, and the final layers are applied to the outputs of all tasks, before splitting into task heads.}
    \label{fig:SubTining-illustration}
\end{figure}

Finetuning a large pretrained model has become a widely used method for achieving optimal performance on a diverse range of machine learning tasks in both Computer Vision and Natural Language Processing~\cite{gpt3, palm, beit, coca}. Traditionally, neural networks are trained ``from scratch'', where at the beginning of the training the weights of the network are randomly initialized. In finetuning, however, we use the weights of a model that was already trained on a different task as the starting point for training on the new task, instead of using random initialization. In this approach, we typically replace the final (readout) layer of the model by a new ``head'' adapted for the new task, and tune the rest of the model (the backbone), starting from the pretrained weights. The use of a pretrained backbone allows leveraging the knowledge acquired from a large dataset, resulting in improved performance on new tasks.


% \fi

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{2-NeurIPS/figure2_new.pdf}
    
    \caption{\textbf{Left.} The \textit{Finetuning Profile} of ResNet-50 Pretrained on ImageNet and finetuned on CIFAR-10. On the x-axis we have 16 res-blocks where each Layer (with Capital L) corresponds to a drop in spatial resolution. \textbf{Middle.} Comparing linear probing, finetuning and SubTuning on CIFAR-10, ResNet-50. Even with few appropriately chosen residual blocks, SubTuning has comparable accuracy to Finetuning. \textbf{Right.} Evaluating SubTuning on \textit{Varying Size} subsets of CIFAR-10. When choosing the right layer, SubTuning shows superior performance for every dataset size. We use logit scale for the y-axis to demonstrate differences across multiple accuracy scales.}
    \label{fig:cifar_resnet_one_block}
\end{figure*}

The finetuning process, while highly effective in improving performance on new tasks, does come with its own set of challenges. One major drawback in the context of multi-task learning \cite{caruana1997multitask, ruder2017overview} is that once the model is finetuned on a new task, its weights may no longer be suitable for the original source task (a problem known as \emph{catastrophic forgetting} \cite{catastrophicforgetting}). Consider for instance the following multi-task setting, which serves as the primary motivation for this paper. Assume we have a large backbone network that was trained on some source task, and is already deployed and running as part of our machine learning system. When presented with a new task, we finetune our deployed backbone on this task, and want to run the new finetuned network in parallel to the old one. This presents a problem, as we must now run the same architecture twice, each time with a different set of weights. Doing so doubles the cost both in terms of compute (the number of multiply-adds needed for computing both tasks), and in terms of memory and IO (the number of bits required to load the weights  of both models from memory). An alternative would be to perform multi-task training for both the old and new task, but this usually results in degradation of performance on both tasks, with issues such as data balancing, parameters sharing and loss weighting cropping up \cite{chen2018gradnorm, sun2020adashare, sener2018multi}. Another option is to use a linear layer, or a small network, on top of the original features, but this typically gives inferior performance compared to finetuning (e.g., see \citet{doimagenet}).

Our objective is therefore to finetune the model for new tasks with minimal added computational power and memory footprint, without sacrificing much in performance on target tasks.
In this work, we study how finetuning can be made more efficient if instead of finetuning all the weights, we finetune only a small subset of intermediate layers. We show that by doing \emph{subset finetuning}, or SubTuning (see~\cref{fig:SubTining-illustration}), we can efficiently deploy new tasks at inference time, with minimal cost in terms of compute, memory and IO.



The key for achieving optimal performance lies in a careful choice of the subset of layers that are finetuned. To do this, we study how each part of the network affects the overall performance as part of the finetuning process. We divide the network into blocks (such as residual blocks in the ResNet architecture or attention layers in a Transformer) and observe how training one block at a time affects the target accuracy (see left side of \cref{fig:cifar_resnet_one_block}). These experiments allow us to draw the \emph{finetuning profile} of the network (see Section~\ref{sec:profile}), which identifies the best consecutive\footnote{We finetune only consecutive blocks as this simplifies our implementation and better utilizes computational resources.} subset of layers to be trained. Interestingly, the optimal subset of layers can be a set of intermediate layers, where the exact choice of layers depends on the dataset, architecture and setting. Simply choosing the layers closest to the output, or otherwise layers with more parameters, may degrade performance. By choosing the best layers in each setting, we are able to achieve performance comparable to full finetuning of the model, with only a small subset of the layers being trained (see \cref{fig:cifar_resnet_one_block} middle).  

We demonstrate the efficiency of our method across different downstream tasks, network architectures (convolutional and transformer based networks) and pretraining methods (supervised and self-supervised) in the vision domain. Importantly, we show how SubTuning lets us deploy a network finetuned for a new task alongside the original backbone network, with minimal additional latency during inference time. We further show that SubTuning achieves superior accuracy compared to full finetuning when training on small datasets (see \cref{fig:cifar_resnet_one_block} right), and that it significantly outperforms competing transfer learning methods such as Head2Toe \cite{head2toe} in a similar setting (see \cref{table:h2t}).
%and that its performance can be further boosted in the Active Learning setting, where we choose to label new unlabeled examples based on the uncertainty of the model. 


\textbf{Our Contributions.}
\begin{itemize}
\item We enhance our understanding of finetuning by introducing the \emph{finetuning profile}, which serves as a crucial tool to illuminate the significance  of different layers during finetuning, as detailed in \cref{sec:profile}.
\item We propose \textbf{SubTuning}, a simple yet effective algorithm that selectively finetunes specific layers based on the \emph{finetuning profile}. We demonstrate its effectiveness and computational efficiency at run-time, as outlined in \cref{sec:computationally_efficient_finetuning}.
\item We investigate the interplay of SubTuning and dataset size, and observe that in low data regimes SubTuning outperforms both linear probing, finetuning and Head2Toe \cite{head2toe}, and show that it can also be used in the active learning setting, as presented in Section~\ref{sec:data}.
\item We conduct a thorough ablation study to investigate the impact of initialization, pruning, and reusing frozen features on the performance of SubTuning, as described in Section~\ref{sec:ablation}.
\end{itemize}



\subsection{Related Work}

\textbf{Multi-Task Learning.} Neural networks are often used for solving multiple tasks. These tasks typically have similar properties, and solving them together allows sharing common features that may capture knowledge that is relevant for all tasks \cite{caruana1997multitask}. However, multi-task learning also presents significant challenges, such as negative transfer \cite{liu2019loss}, loss balancing \cite{lin2022a, michel2022balancing}, optimization difficulty \cite{mtl-optimization}, data balancing and shuffling~\cite{purushwalkam2022challenges}. While these problems can be mitigated by careful sampling of the data and tuning of the loss function, these solutions are often fragile \cite{worsham2020multi}. In a related setting called \emph{Continual Learning} \cite{rusu2016progressive, rebuffi2017icarl, kirkpatrick2017overcoming, kang2022class}, adding new tasks needs to happen on-top of previously deployed tasks, while losing access to older data due to storage or privacy constraints, complicating matters even further. 



\textbf{Parameter Efficient Transfer Learning.}
In recent years, it became increasingly popular to finetune large pretrained models~\cite{bert, clip, masked}. As the popularity of finetuning these models grows, so does the importance of deploying them efficiently for solving multiple tasks. Thus there has been a growing interest, especially in the NLP domain, in Parameter Efficient Transfer Learning (PETL)~\cite{progressive, lst, head2toe, sidetuning, howfine, piggyback, bitfit, model_adaptation} 
where we either modify a small number of parameters, add a few small layers or mask~\cite{Maskingalternative} most of the network. Using only a fraction of the parameters for each task can help in avoiding catastrophic forgetting and can be a good solution for both multi-task learning and continual learning. These methods include Prompt Tuning~\cite{prefix-tuning, prompt-tuning, visual-prompt-tuning}, adapters~\cite{adapters-nlp, residual_adapters, adapters-conv,parallel-adapters}, LoRA~\cite{lora}, sidetuning~\cite{sidetuning}, feature selection~\cite{head2toe} and masking~\cite{howfine}. \citet{fu2022effectiveness} and \citet{he2021towards} (see also references therein) attempt to build a unified approach of PETL and suggest improved methods. 

Our work draws inspiration from the PETL literature, and to some extent shares the core motivations of the papers mentioned above. That said, many of the PETL works operate in the NLP domain, where using models with billions of parameters has become a common practice, and hence their main objective is reduction in parameter count. Our work focuses on deployment of networks for computer vision, which are typically much smaller in terms of parameters, and so our primary focus is on the \emph{computational efficiency} of the deployed model, rather than on its parameter efficiency. While some of the works above suggest methods that can also improve computational efficiency,  unlike previous work, our approach is versatile and can be applied and appended to any architecture, and does not assume sparsity optimized hardware. 
Finally, our \emph{finetuning profiles} offer unique insight into the mechanisms of finetuning, making our research not only practical but also scientifically illuminating. We also note that SubTuning is compatible with many other PETL methods, and composing SubTuning with methods like LoRA and Head2Toe is a promising research direction that we leave for future work.

In a recent study, \citet{percy-surgical} investigated the impact of selective layer finetuning on small datasets and found it to be more effective than traditional finetuning. They observed that the training of different layers produced varied results, depending on the shifts in data distributions. Specifically, they found that when there was a label shift between the source and target data, later layers performed better, but in cases of image corruption, early layers were more effective.

While our work shares some similarities with \citet{percy-surgical}, the motivations and experimental settings are fundamentally different. Primarily, our research focuses on multi-task learning and aims to develop an efficient finetuning algorithm that can achieve high performance, while \citet{percy-surgical} focuses on improved finetuning for small corrupted datasets. Additionally, \citet{percy-surgical} finetunes large parts of the network, while in our work we finetune a carefully selected minimal subset of the layers.


%In addition, we extend our analysis to scenarios with more data and show that SubTuning is a viable method even in these cases. By examining the performance of individual ResBlocks, we also construct the ``Finetuning Profile," which sheds new light on the relationship between the layer finetuned and the downstream performance.




\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth,trim={0 1.2cm 0 0}]{2-NeurIPS/finetune_profiles.pdf}
    \caption{Finetuning profiles for different architectures, initializations and datasets.}
    \label{fig:finetuning_profiles}
\end{figure*}



==> 2-NeurIPS/sections/the_finetuning_profile.tex <==




